Hot-spots around Sagittarius A*: Joint fits to astrometry and polarimetry

Observations of Sagittarius A* (Sgr A*) in near-infrared (NIR) show irregular flaring activity. Flares coincide with astrometric rotation of brightness centroid and with looping patterns in fractional linear polarization. These signatures can be explained with a model of a bright hot-spot, transiently orbiting the black hole. We extend the capabilities of the existing algorithms to perform parameter estimation and model comparison in the Bayesian framework using NIR observations from the GRAVITY instrument, and simultaneously fitting to the astrometric and polarimetric data. Using the numerical radiative transfer code ipole, we defined several geometric models describing a hot-spot orbiting Sgr A*, threaded with magnetic field, and emitting synchrotron radiation. We then explored the posterior space of our models in the Bayesian framework with a nested sampling code dynesty. We have used 11 models to sharpen our understanding of the importance of various aspects of the orbital model, such as non-Keplerian motion, hot-spot size, and off-equatorial orbit. All considered models converge to realizations that fit the data well, but the equatorial super-Keplerian model is favored by the currently available NIR dataset. We have inferred an inclination of ~ 155 deg, which corroborates previous estimates, a preferred period of ~ 70 minutes, and an orbital radius of ~ 12 gravitational radii with the orbital velocity of ~ 1.3 times the Keplerian value. A hot-spot of a diameter smaller than 5 gravitational radii is favored. Black hole spin is not constrained well.

==> copied_old_text.tex <==

%The model IDs, as given in Table~\ref{tab:models} are chosen to convey the most important information about each model. The first tag refers to the Keplerianity of the orbit, with 3 possible values: fixed Keplerian orbital speed (K), sub- and super- orbital speeds (subK and supK respectively).


%We have performed parameter estimation using 11 different models listed in Table \ref{tab:models}. The models have been constructed to probe different aspects of the importance of the parameters while keeping enough similarities to be comparable. The model IDs are chosen to convey the most important information about each model. The first tag refers to the Keplerianity of the orbit, with 3 possible values: fixed Keplerian orbital speed (K), sub- and super- orbital speeds (bK and pK respectively). For not fixed cases(bK, pK) we search for the best fitted value of $K_{\textrm{coeff}}$. Next, is the tag regarding magnetic field orientation in a fixed vertical topology: the default mode (db) refers to the field polarity aligned with the spin axis of the black hole, pointing away from the observer for $i>90^\circ$, and the flipped one is the opposite to that. The last tag refers to more specific parameter investigations: (a0) describes models with fixed spin value ($a_*=0$), and (pa180) models with fixed position angle ($PA=180$~deg). For the last three models instead of fixing a parameter to a specific value we have added extra ones, where (ss) refers to spot size which is also a high resolution run at $192\times192$, since for smaller spots higher resolution is required, (BG) refers to an extra parameter added to emulate constant emission from the background (the accretion disc) and it's aim is to test the assumption made in \citetalias{G23} that the bulk of total intensity should be produced in the disk rather than the spot. The last model has 3 extra parameters (th\_ofst), and is the most complex model, allowing for spots to move in off-equatorial trajectories. It \monika{Our algorithm} \ar{It's only for this model} also allows for the black hole to be off-center in the astrometry plot. Only the first 4 models are presented here, with the exploratory runs discussed in Conclusions and Appendices \ref{app:ss}-\ref{app:th}



%The first test is with models K\_db and K\_fb and it aims to distinguish any preference between the two possible magnetic field orientations of vertical geometry. The results are visible in Fig. \ref{fig:corner_K}. The top panel presents the corner (or triangle) plot of the fit, with 1D and 2D posterior distributions. The printed values are the peak of each distribution with $1\,\sigma$ margins. Black lines denote the values of the highest likelihood run. The bottom panels show polarimetry and astrometry using those highest-likelihood parameters. 

%The key parameters, reported in Table \ref{tab:models}, as well as the posteriors are similar between the two models. Additionally, the evidence $\log(Z) \sim -23$ close for both runs strengthens the hypothesis of indifferent $B_{\text{field}}$ orientation in NIR. Inclination $i=155 \pm 5$ deg and spot's radius $r_s=10\,$M is compatible with estimations from \citetalias{G23} ($155$ deg and $9\,$M respectively). Spin parameter $a_*$ is unconstrained, as well as $\phi_{cam}$, since it is defined in Kerr-Schild coordinates and thus correlated with spin and $r_s$ in order for  There is one surprising result regarding PA, where the models converge to $PA=130 \pm 20$ deg, which is different than $PA=180$ deg reported in \citetalias{G23}. This arises from the simultaneous fit of polarimetry and astrometry rather than fitting only astrometry, since polarimetry is more sensitive to PA (due to the inner loop rotating in Q,U space). The effect of PA is further discussed in Apendix~\ref{app:pa180}. This best-bet parameters corresponds to period $P\sim70$ min, slightly larger than \citetalias{G23} that found a period of $P=60$ min. The total $\chi_{\textrm{eff}}^2$ for both models is calculated at $\chi_{\textrm{eff}}^2 = 0.6 $ verifying a successful fit.   

%First feature to note is that the posteriors between the two $B_{\textrm{field}}$ orientations look identical, as well as the light-curves, also reflected in the close values of log-Evidence, $\log(Z)\sim -23$ with the flipped case 0.7 smaller. This meets our expectations as noted in Section \ref{sec:methods}, since Faraday effects are negligible in NIR frequencies\monika{the linear polarization fitted here is identical (or something like that), you can also refer to Jesse paper where we check all this stuff in the appendix}. 
%Next, the inclination $i=155 \pm 5$ deg is in good agreement with \citetalias{G23} and \citetalias{Y24}. The posteriors on spin look completely unconstraining, and the high values of $B_{\textrm{field}}$ strength verify our assessment, that thermal electrons need a very energetic environment to produce radiation at NIR frequencies. 
%The radius peaks at $r_s=10$M larger than the value reported in \citetalias{G23}, but the posterior overlaps with their value of $r_s=9$M. Then $\phi_{\textrm{cam}}$ that controls the starting point of the spot on the sky also appears unconstrained, but this is due to a correlation with spin, meaning for different values of spin, different values of $\phi_{\textrm{cam}}$ are needed to keep the spot at the same position\monika{a and phicam do not seem to be correlated in the triangle plot}. \ar{its hard to tell cause they're messy.} Lastly, $LP_{\textrm{frac}}$, that controls the fraction of linear polarization is well confined around $0.20$, but more importantly PA is also well constrained around $130 \pm 20$ deg, which is different than PA=180 reported in \citetalias{G23}. This arises from the simultaneous fit of polarimetry and astrometry rather than fitting only astrometry, since polarimetry is more sensitive to PA (due to the inner loop rotating in Q,U space). The effect of PA is further discussed in Apendix \ref{app:pa180}. This set of parameters corresponds to period $P\sim70$ min, slightly larger than \citetalias{G23} that found a period of $P=60$ min. The total $\chi_{\textrm{eff}^2}$ for both models is calculated at $\chi_{\textrm{eff}}^2 = 0.6 $ verifying a successful fit. 


%The other pair of models we discuss in this section are supK\_db and subK\_db that aim to answer whether a hot-spot has a preferred orbital speed. These models have been created identical, with only distinction the range of $K_{\textrm{coeff}}$ and $r_s$ being $(0.5-1)$ and $(7-14)$ for subK\_db and $(1-1.5)$ and $(8-15)$ for supK\_db. The results can be seen in Fig. \ref{fig:corner_nK} which is laid out in the same way as Fig. \ref{fig:corner_K}. The values for inclination, $B_{\textrm{field}}$, $LP_{\textrm{frac}}$ and PA remain very similar with the Keplerian fit. The ambiguity in spin values persists leading to the same effect for $\phi_{\textrm{cam}}$. Naturally, differences appear in the posteriors of $r_s$ and $K_{\textrm{coeff}}$, since the priors for $K_{\textrm{coeff}}$ are disjoint. Model supK\_db has a mean value of $r_s = 12.66$, considerably larger than the Keplerian models and \citetalias{G23}. This is accompanied by $K_{\textrm{coeff}} = 1.33$, meaning orbital velocity $33\%$ higher than the Keplerian, leading to a similar orbital period of $P=72$ min. For the subK\_db model, the differences are not so prominent, with both $r_s$ and $K_{\textrm{coeff}}$ close to Keplerian values, $r_s=9.6$, $K_{\textrm{coeff}}=0.92$. Both posteriors exhibit uneven distributions towards Keplerian values, particularly visible in the case of $K_{\textrm{coeff}}$. The orbital period remains $P=70$ min. Attempting a model selection by comparing the Evidence of these 3 models (K\_db, subK\_db, supK\_db) the super-Keplerian velocities are favored, with $log(Z)=-21.9$, more than 2 larger than the sub-Keplerian counterpart and 1 than the Keplerian model. This is further supported by the $\chi_{\textrm{eff}}^2$ values, $\chi_{\textrm{eff}}^2 = 0.4$ and $\chi_{\textrm{eff}}^2=0.9$ for supK\_db and subK\_db respectively.      

%\monika{this section, especially the second part is very difficult to read because all numbers are reported in text. I think it would be maybe useful to expand table 2 and put these a couple of essential parameters into it. and the text maybe should focus on comparisons between first 4 models:are there common parameters (rs, inc, P)? is Keplerian or super/subKeplerian more preferred? which models have lower chi2 and highest evidence?}
%==========
%==========
\section{Conclusions}
\label{sec:conclusions}
%=============

We have created a family of semi-analytic models of a bright orbiting spot to fit Sgr~A* NIR data reported by GRAVITY in \citetalias{G23}. The analysis is novel to what has been done before by fitting polarimetry and astrometry simultaneously. It also accommodates for an extra degree of freedom, being $K_{\textrm{coeff}}$ with important implications for the accretion flow, as well as the creation and exact location of the spot. A further analysis on effects of specific parameters (such as spin and PA) is reported in Appendices. Overall the present work aims to perform a more dedicated parameter estimation from the given dataset, utilizing the widely accepted hot-spot model. 

All models showcased consistency in inclination and position angle ($i=155$~deg and $PA=130$~deg). The former in agreement to various previous works (cite), but not the later. Unanimously models pointed to $PA\sim130$ which is $50$ deg lower than \citetalias{G23} and \citetalias{Y24}. In Appendix \ref{app:pa180} we report a run with models identical to supK\_db and subK\_db but fixing $PA=180$ deg. The quality of the fit deteriorates significantly, strengthening the fiducial PA estimation. 

In contrast, the spin posteriors are not constraining for any model with their posteriors almost uniform. This is further supported in Appendix \ref{app:a0}, where the pipeline is run with fixed spin value, $a_*=0$. The results, remain unaltered with equal values for $\log(Z)$, pointing to an irrelevant parameter for this fit. This is an interesting finding, given the same pipeline used in \citetalias{Y24} showed a preference for high spins, $a_* \sim 0.9$. The primary difference is data quality, in terms of cadence and errors. In \citetalias{Y24} it was argued that the predominant effect of spin to light curves arises from the secondary image which is a rather subtle feature of the system, requiring fine data to capture. 

The next model from the exploratory runs, visible in Appendix \ref{app:BG}, was made to test the assumption made in \citetalias{G23}, that the background emission should dominate total intensity. In our main models we considered that the majority of radiation should come from the spot, using two arguments, one model driven and one data driven. 1) The thermal electrons of the disk should produce weak radiation in NIR frequencies, in contrast to the hot-spot that should consist of highly energetic, non-thermal electrons. 2) As presented in \cite{gravity:2020c}, the total flux during flares can increase up to 2 orders of magnitude, meaning the background, or the disk, is strongly subdominant to the hot-spot, that is believed to cause these strong spikes in total intensity. So, to test this argument we create a model with an extra parameter, emulating a constant background component of Stokes I. The parameter $I_{BG}$ is a scaling factor with respect to the peak emission of the spot during a full orbit, i.e. $I_{\textrm{tot}}=I_{\textrm{spot}}+I_{BG}*\textrm{max}(I_{\textrm{spot}})$. That means $I_{BG}=1 $ translates to a disk with equal intensity as the spot at its peak. The results are visible in Fig. \ref{fig:corner_bg}. The posterior for $I_{BG}$ lays at $I_{BG}=2 \pm 2$. As expected though, it is strongly correlated with $LP_{\textrm{frac}}$, and the most reasonable values of $LP_{\textrm{frac}}<0.5$ yield values of $I_{BG}<1$. Indicatively, the highest likelihood model, has $LP_{\textrm{frac}}=0.24$, similar to all main models and $I_{BG}=0.15$, making background emission $\sim6$ times dimmer than the hot-spot.           
   
The model that performed best was supK\_db placing the spot at $r_s ~ 12.5$ M with an orbital coefficient $K_{\textrm{coeff}} = 1.33$. An image of the spot on the sky can be seen in the top panel of Fig. \ref{fig:movie109_256}. That is a compelling result since there have not been any works reporting such velocities from the mid plane of accretion disks, raising the question if the mid-plane is the correct location to explain NIR hot-spots. A similar trajectory in the jet sheath could be more plausible, since this is the region separating the main disk and then jet , where velocities can easily exceed their Keplerian equivalent for a trajectory with the same $r_s$ on the mid-plane. Similar arguments have been made in models of \cite{ball:2021,Lin2023,Aimar2023}.   \citet{Antonopoulou2024} also concluded preference for superkeplerianity in case of equatorial orbits.

 To test this hypothesis we performed another exploratory test, supK\_db\_th\_ofst which is presented in Appendix \ref{app:th}. This model has an extra parameter ($\theta_s$), being the polar angle of the spot's orbit. There are two main findings from this analysis, 1) the overall fit performance deteriorates with the inclusion of non-equatorial orbits, with $\log(Z)=-24$, instead of $\log(Z)=-22$ from fiducial models; 2) There is an acceptable solution for all $\theta_s$ values ($45-90$ deg), with the posterior of $\theta_s$ fairly uniform. Despite that second point, the solutions with $\theta_s < 80 $ can be considered disfavored, given the shape of their polarimetry light-curves that are not circular, but rather crescent like, see bottom panels of Fig. \ref{fig:corner_th}. The above analysis adds an extra degree of complexity on the discussion of spot origin and location, since orbital velocities point to off-equatorial trajectories, but with polarimetry equatorial spots appear more plausible. Perhaps this is a forecast of the circular character the data obtained after the averaging tecnique.  

Further progress on understanding the flaring in Sgr~A* should be enabled by obtaining additional high quality data sets both in NIR and millimeter bands. A particularly important constraints could be provided by simultaneous observations of NIR polarimetry and astrometry with millimeter polarimetry for the flaring source. Moreover, developing very long baseline interferometric arrays may provide millimeter wavelength relative astrometry along with snapshot imaging of the flaring source \citep{ngeht2023, Emami2023}.
